Robust Performance Analysis for Time-Varying Multi-Agent Systems with Stochastic Packet Loss

Recently, a scalable approach to system analysis and controller synthesis for homogeneous multi-agent systems with Bernoulli distributed packet loss has been proposed. As a key result of that line of work, it was shown how to obtain upper bounds on the $H_2$-norm that are robust with respect to uncertain interconnection topologies. The main contribution of the current paper is to show that the same upper bounds hold not only for uncertain but also time-varying topologies that are superimposed with the stochastic packet loss. Because the results are formulated in terms of linear matrix inequalities that are independent of the number of agents, multi-agent systems of any size can be analysed efficiently. The applicability of the approach is demonstrated on a numerical first-order consensus example, on which the obtained upper bounds are compared to estimates from Monte-Carlo simulations.

==> doc/header.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}

\makeatletter
\let\old@ssect\@ssect % Store how ifacconf defines \@ssect
\makeatother

\usepackage{natbib}
\usepackage{csquotes}
\usepackage[bookmarks=false]{hyperref}

\makeatletter
\def\@ssect#1#2#3#4#5#6{%
    \NR@gettitle{#6}% Insert key \nameref title grab
    \old@ssect{#1}{#2}{#3}{#4}{#5}{#6}% Restore ifacconf's \@ssect
}
\makeatother

% Math related packages
\usepackage{amsmath, amssymb}
\usepackage{mathtools}
\usepackage{commath}
\usepackage[casesstyle, subnum]{cases}

% For underbar
\usepackage{accents}

% Better lists and tables
\usepackage{booktabs}
\usepackage{enumitem}

% Draw vector graphics and plots
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}

\usetikzlibrary{
 	arrows.meta,                                          % Proper arrow tips
  	calc,                                                 % Support for calculating positions
  	positioning,                                          % Better support for relative positioning
  	patterns
}

\usepgfplotslibrary{fillbetween}
\pgfplotsset{
    compat=1.17,
    cycle list name=linestyles*,
    every axis plot/.append style={
        thick
    },
}

% Introduce underbar
\DeclareRobustCommand{\ubar}[1]{\underaccent{\bar}{#1}}

% Useful math shortcuts
\newcommand{\bbma}{\begin{bmatrix}}
\newcommand{\ebma}{\end{bmatrix}}
\newcommand{\real}{\mathbb{R}}

\DeclareMathOperator{\expect}{\mathbb{E}}
\DeclareMathOperator{\probab}{Pr}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}

